EMG Tokenization Preserves Movement Information at a Fraction of the Bitrate

Wireless electromyography (EMG) interfaces must balance electrode coverage against transmission bandwidth. Here, we show that compact EMG tokens substantially reduce payload while retaining information for three-dimensional hand-pose decoding. We evaluate two causal tokenizers fitted without pose labels: an encoder pretrained to reconstruct EMG spectra and one based on SPAR, an engineered spectral-spatial representation of neighbouring electrodes. In personalized, within-session experiments with 320-channel EMG from nine participants, we compare tokenized and continuous features using matched decoder architectures and training procedures. Averaged across decoders, tokenization changed mean error by +0.01 mm for SPAR (95% confidence interval: -0.12 to 0.14) and +0.45 mm for the learned representation (0.10 to 0.82). Both increases met a 1 mm non-inferiority criterion. Stored token arrays reduced payloads 41-fold relative to raw EMG and 36-fold relative to continuous SPAR features. On sampled windows of the public emg2pose benchmark's test partition, absolute differences in mean error between learned tokens and continuous features were below 0.05 mm across 176 participants and in the subset of 20 participants unseen during training. Electrode coverage, calibration, and unseen recordings affected SPAR decoding more than quantization did. In a computational benchmark, optimized SPAR generated tokens for 63 channels within 20 ms on a Cortex-M55 microcontroller. These findings support tokenization as a compact interface between wearable sensing and movement decoding, allowing decoders to be updated while the wearable encoder and transmitted representation remain fixed.

==> xref-main.tex <==
\newlabel{M-sec:introduction}{{I}{1}{Introduction}{}{}}
\newlabel{M-sec:method}{{II}{1}{Methods}{}{}}
\newlabel{M-fig:concept}{{1}{2}{\textbf {From high-density electromyography (EMG) recordings to a transmittable representation.} \textbf {A:} Nine participants performed individual finger movements, grasping, and two- and three-finger pinches. Markerless hand tracking was recorded alongside surface EMG (sEMG) from 320 electrodes distributed across five grids. The lower band illustrates an eight-channel subset obtained by selecting every 40th channel from the 320-channel recording. \textbf {B:} Continuous EMG features and discrete tokens are used to train three-dimensional (3D) hand-pose decoders on a high-performance computing (HPC) system. Their decoding errors are compared using the same decoder architecture and training procedure within each pair. \textbf {C:} An assumed Bluetooth LE (BLE) 2M application throughput of 1.4\,Mbit/s \citep {bluetoothsigLEprimer} supports up to 42 channels of raw 16-bit EMG at 2,048\,Hz, and the 43rd exceeds the budget. Packed 10-bit tokens at 50\,Hz would support 2,800 channels. These are payload-only calculations before application packet headers, not measured transmission or computational capacities (Section~\ref {S-app:bandwidth}; Fig.~\ref {S-fig:operating-points}; Supplementary Data~1)}{}{}}
\newlabel{M-fig:learned-tokenizer}{{2}{3}{\textbf {Learned electromyography (EMG) tokenizer and intermediate representations.} \textbf {A:} A shared encoder processes 160\,ms EMG windows every 20\,ms. Four residual blocks extend the receptive field to 480\,ms, while a fixed codebook maps each 256-dimensional output to one of 1,024 tokens (10 bits). Layer dimensions such as \(32\rightarrow 256\) denote the input and output feature dimensions. Conv1D denotes a one-dimensional convolution, GELU the Gaussian error linear unit, LayerNorm layer normalization, and L2 the Euclidean distance. \textbf {B:} Example normalized EMG waveform spanning 480\,ms (participant 1, electrode 1). \textbf {C:} Three of the 256 intermediate features (indices 1, 128, and 256) after the second residual block, shown at nine consecutive time points spaced 20\,ms apart. \textbf {D:} The resulting 256-dimensional feature vector, mapped to token identifier (ID) 93. Time zero in C corresponds to 480\,ms in B}{}{}}
\newlabel{M-fig:spar-patch}{{3}{3}{\textbf {Neighbourhoods and boundary handling of the spectral--spatial representation.} Grey marks the centre electrode, red the horizontal and vertical neighbours, and blue the auxiliary electrode. At a boundary, an electrode on the opposite side of the centre replaces the missing neighbour (dashed arrow), and its coupling is set to zero after the matrix logarithm. Each band contributes the centre's diagonal entry and the real horizontal and vertical couplings}{}{}}
\newlabel{M-eq:spar-matrix}{{1}{3}{SPAR: spectral--spatial features and tokenization}{}{}}
\newlabel{M-sec:experiments}{{\mbox  {II-D}}{4}{Evaluation protocol}{}{}}
\newlabel{M-sec:representation}{{\mbox  {II-G}}{4}{Representation visualization and pose retrieval}{}{}}
\newlabel{M-sec:stats}{{\mbox  {II-I}}{5}{Outcomes and statistical analysis}{}{}}
\newlabel{M-sec:results}{{III}{5}{Results}{}{}}
\newlabel{M-fig:dpose-main}{{4}{6}{\textbf {Hand-pose decoding accuracy, computational cost, and quantization effects.} \textbf {A:} Unfiltered three-dimensional (3D) error over 20 wrist-relative landmarks, decoder parameters including frozen backbones, and 32-bit floating-point (FP32) decoder latency. Qwen3 \citep {qwen3technicalreport} and TabPFN \citep {hollmann2025tabpfn,priorlabs2026tabpfn35} are frozen pretrained decoders, and TCN is a temporal convolutional network. Grey points are participant means over three seeds, and coloured symbols group means. Latency is the mean and standard deviation per complete-pose prediction (batch size one, RTX 4090), excluding feature extraction and tokenization (TabPFN also includes host-processor work). Dashed lines mark the 20\,ms update interval and the retrained convolutional neural network (CNN) from IEEE Transactions on Biomedical Engineering (TBME CNN) \citep {simpetruLearningHandModel2024}. Brackets compare the spectral--spatial representation (SPAR) with learned tokens in the proposed decoder (*, \(p=0.016\)) and SPAR tokens with the adapted CNN (< 1\,mm, \(p=0.016\)). \textbf {B:} Stored-array payload for 320 channels before packet headers. The dashed line marks the assumed Bluetooth LE (BLE) 2M throughput of 175\,kB/s \citep {bluetoothsigLEprimer}. Labels give stored types: unsigned (uint16) and signed (int16) 16-bit integers for tokens and raw electromyography (EMG), and FP32 for features. \textbf {C:} Token error minus continuous-feature error. Circles are participants, diamonds are means, and bars are 95\% confidence intervals. Bold Pooled rows average the differences across decoders within each tokenizer, and both upper 95\% confidence limits lie below the dashed 1\,mm bound (\(p=0.016\) each). The four \(p\)-values in A and C are from exact paired sign-flip permutation tests, Holm-adjusted together (Section~\ref {sec:stats})}{}{}}
\newlabel{M-fig:decoding}{{5}{7}{\textbf {Decoded hand movements and movement-specific errors.} \textbf {A:} Example predictions from participant 6. Traces span 4\,s, and scoring uses the final second of each predefined test window. Black indicates measured movement, red spectral--spatial representation (SPAR) tokens, and dashed blue continuous SPAR. Predictions are smoothed with a causal One Euro filter for display only. Traces show the thumb-tip-to-pinky-base distance for the thumb, the fingertip-to-wrist distance for the other digits (its mean over fingertips for the fist), and the thumb-to-fingertip distance for the pinches (averaged over index and middle fingers for the three-finger pinch). Section~\ref {S-app:noise} describes the predictions shown between scored seconds and the filter. \textbf {B:} Unfiltered three-dimensional (3D) error across 20 landmarks for each movement, averaged over nine participants and three seeds. Bars show group means with 95\% confidence intervals, and diamonds identify participant 6. Supplementary Data~2 reports the paired comparisons}{}{}}
\newlabel{M-sec:manifold}{{\mbox  {III-B}}{7}{SPAR tokens retain hand pose across repetitions}{}{}}
\newlabel{M-fig:token-pose}{{6}{8}{\textbf {Hand-pose structure in spectral--spatial representation (SPAR) token space.} \textbf {A--C:} One three-dimensional Uniform Manifold Approximation and Projection (UMAP) of participant 1's token histories across eight movements. Each movement is projected separately onto its mean-trajectory plane and repositioned for display (Section~\ref {sec:representation}). Figure~\ref {S-fig:token-history} shows how the projected trajectories change as token history increases from a single update to 960\,ms. \textbf {A:} Movement identity, with icons indicating the active fingers. \textbf {B:} Hand closure normalized separately for each movement. \textbf {C:} Phase-aligned, smoothed repetitions (thin) and their mean trajectory (thick), with cycle starts near the open-hand pose (dots) and traversal direction (arrows). \textbf {D:} Pose retrieval for single updates in the test windows, matched against repetitions outside the training windows, using continuous SPAR, dequantized tokens, or token identifiers (IDs) in the original representation space. Thin lines show the nine participants and the thick line their mean. Dashed lines are descriptive references: disrupted token--pose alignment (11.3\,mm, a mean of participant medians, for which 1,024-code tokens give 7.3\,mm) and matching using measured poses (4.4\,mm). The curves and the pose-space reference are phase-balanced means. Asterisks indicate increases over continuous SPAR (exact paired permutation (sign-flip) tests, Holm-adjusted across three comparisons; \(p=0.043\), \(0.016\), and \(0.012\)). Retrieval, display-selection rules, and reference construction are detailed in Section~\ref {S-app:manifold}}{}{}}
\newlabel{M-fig:stm32n6}{{7}{9}{\textbf {Computational performance of electromyography (EMG) tokenization on a Cortex-M55 microcontroller.} The spectral--spatial representation (SPAR) implementations were tested at 600\,MHz with synthetic 2\,kHz EMG. Timing includes windowing, normalization, feature extraction, codebook search, and token packing, but excludes acquisition, radio transmission, and pose decoding. \textbf {A:} Median compute time per update over 16 timed updates, after 16 untimed warm-up updates. Open symbols and dashed lines show the original C implementations, and filled symbols and solid lines the optimized ones. Every timed update at the marked SPAR channel limits met the 20\,ms interval. \textbf {B:} Optimized SPAR time per channel by processing stage, with labels giving values at 320 channels. The dashed line shows time per channel from a linear fit of total time against channel count through the origin (Section~\ref {S-app:n6})}{}{}}
\newlabel{M-sec:sensitivity}{{\mbox  {III-D}}{9}{Sensitivity to noise, electrode loss, calibration, and unseen recordings}{}{}}
\newlabel{M-LastPage}{{V}{11}{Acknowledgment}{}{}}

